A Study of Newly Observed Hostnames and DNS Tunneling in the Wild

The domain name system (DNS) is a crucial backbone of the Internet and millions of new domains are created on a daily basis. While the vast majority of these domains are legitimate, adversaries also register new hostnames to carry out nefarious purposes, such as scams, phishing, or other types of attacks. In this paper, we present insights on the global utilization of DNS through a measurement study examining exclusively newly observed hostnames via passive DNS data analysis. We analyzed more than two billion such hostnames collected over a period of two months. Surprisingly, we find that only three second-level domains are responsible for more than half of all newly observed hostnames every day. More specifically, we found that Google's Accelerated Mobile Pages (AMP) project, the music streaming service Spotify, and a DNS tunnel provider generate the majority of new domains on the Internet. DNS tunneling is a covert channel technique to transfer arbitrary information over DNS via DNS queries and answers. This technique is often (ab)used by attackers to transfer data in a stealthy way, bypassing traditional network security systems. We find that potential DNS tunnels cause a significant fraction of the global DNS requests for new hostnames: our analysis reveals that nearly all resource record type NULL requests and more than a third of all TXT requests can be attributed to DNS tunnels. Motivated by these empirical measurement results, we propose and implement a method to identify DNS tunnels via a step-wise filtering approach that relies on general characteristics of such tunnels (e.g., number of subdomains or resource record type). Using our approach on empirical data, we successfully identified 273 suspicious domains related to DNS tunnels, including two known APT campaigns (Wekby and APT32).

==> tables/top10_domains_example.tex <==
\begin{tabular}{@{}lll@{}}
\toprule
Domain name      & Count     & Share   \\ \midrule
ampproject.net   & 5.829.683 & 20.25\% \\
1yf.de           & 4.114.835 & 14.3\%  \\
53.de            & 3.374.212 & 11.72\% \\
spotilocal.com   & 2.958.028 & 10.28\% \\
8u6.de           & 2.225.447 & 7.73\%  \\
mts.ru           & 1.128.178 & 3.92\%  \\
imrworldwide.com & 475.190   & 1.65\%  \\
beeline.ru       & 388.343   & 1.35\%  \\
cnr.io           & 367.542   & 1.28\%  \\
dotnxdomain.net  & 354.581   & 1.23\%  \\ \bottomrule
\end{tabular}
